Observational Signatures of a Previous Dynamical Instability in Multi-planet M-Dwarf Systems

We identify observational signatures suggesting a history of dynamical instability in 26 out of 34 M-dwarf multi-planet systems containing no large planets. These systems may have primarily formed in a gas-rich environment, potentially hosted more planets and were more compact. We extend previous simulations of the formation of the TRAPPIST-1 system to 100 Myr to test the stability of these systems without gas. We find the absence of a strong mean motion resonance in the innermost planet pair and the absence of three body resonances throughout the system are likely to result in the merging and ejection of planets after the gas disk disperses. The runs that experience such an instability tend to produce final systems with lower multiplicities, period ratios larger than two, increased orbital spacings, higher planetary angular momentum deficits, and slightly smaller mass ratios between adjacent planets. Remarkably, we find these same trends in the observations of M-dwarf multi-planet systems containing no large planets. Our work allows us to identify specific systems that may have experienced an instability and suggests that only ~25% of these systems formed in their current observed state while most systems were likely more compact and multiplicitous earlier in time. Previous research indicates that systems that have experienced a late stage giant impact may host planets potentially more habitable than the systems that did not. With this in mind, we suggest systems around M-dwarfs that contain period ratios larger than two be given priority in the search for habitable worlds.

==> obs_data.tex <==
\clearpage
\begin{turnpage}


\begin{table}

\caption{Observational data used in our study.}
\label{tab:obs_data}
\centering
\begin{tabular}{lrrlrllllll}
\toprule
Hostname & $M_{\star}/M_{\odot}$ & no. planets & planet name & planet orb per (days) & planet $m / M_{\oplus}$ & planet $m$sin$i\, / M_{\oplus}$ & pl $r / R_{\oplus}$ & $+\sigma_1$ pl $r / R_{\oplus}$  & Approximate $m/M_{\oplus}$ & Class \\
\midrule
TRAPPIST-1 & 0.090 & 7 & TRAPPIST-1 b & 1.511 & 1.374 & - & 1.116 & 0.014 & - & Small PR \\
TRAPPIST-1 & 0.090 & 7 & TRAPPIST-1 c & 2.422 & 1.308 & - & 1.097 & 0.014 & - & Small PR \\
TRAPPIST-1 & 0.090 & 7 & TRAPPIST-1 d & 4.049 & 0.388 & - & 0.788 & 0.011 & - & Small PR \\
TRAPPIST-1 & 0.090 & 7 & TRAPPIST-1 e & 6.101 & 0.692 & - & 0.920 & 0.013 & - & Small PR \\
TRAPPIST-1 & 0.090 & 7 & TRAPPIST-1 f & 9.208 & 1.039 & - & 1.045 & 0.013 & - & Small PR \\
TRAPPIST-1 & 0.090 & 7 & TRAPPIST-1 g & 12.352 & 1.321 & - & 1.129 & 0.015 & - & Small PR \\
TRAPPIST-1 & 0.090 & 7 & TRAPPIST-1 h & 18.773 & 0.326 & - & 0.755 & 0.014 & - & Small PR \\
Teegarden's Star & 0.100 & 3 & Teegarden's Star b & 4.906 & - & 1.160 & - & - & - & Big PR \\
Teegarden's Star & 0.100 & 3 & Teegarden's Star c & 11.416 & - & 1.050 & - & - & - & Big PR \\
Teegarden's Star & 0.100 & 3 & Teegarden's Star d & 26.130 & - & 0.820 & - & - & - & Big PR \\
GJ 1002 & 0.120 & 2 & GJ 1002 b & 10.347 & - & 1.080 & - & - & - & Big PR \\
GJ 1002 & 0.120 & 2 & GJ 1002 c & 21.202 & - & 1.360 & - & - & - & Big PR \\
GJ 1061 & 0.120 & 3 & GJ 1061 b & 3.204 & - & 1.370 & - & - & - & Big PR \\
GJ 1061 & 0.120 & 3 & GJ 1061 c & 6.689 & - & 1.740 & - & - & - & Big PR \\
GJ 1061 & 0.120 & 3 & GJ 1061 d & 13.031 & - & 1.640 & - & - & - & Big PR \\
Kepler-42 & 0.130 & 3 & Kepler-42 b & 1.214 & - & - & 0.780 & 0.220 & 0.423 & Big PR \\
Kepler-42 & 0.130 & 3 & Kepler-42 c & 0.453 & - & - & 0.730 & 0.200 & 0.358 & Big PR \\
Kepler-42 & 0.130 & 3 & Kepler-42 d & 1.865 & - & - & 0.570 & 0.180 & 0.141 & Big PR \\
YZ Cet & 0.140 & 3 & YZ Cet b & 2.021 & - & 0.700 & - & - & - & Small PR \\
YZ Cet & 0.140 & 3 & YZ Cet c & 3.060 & - & 1.140 & - & - & - & Small PR \\
YZ Cet & 0.140 & 3 & YZ Cet d & 4.656 & - & 1.090 & - & - & - & Small PR \\
GJ 3323 & 0.160 & 2 & GJ 3323 b & 5.364 & - & 2.020 & - & - & - & Big PR \\
GJ 3323 & 0.160 & 2 & GJ 3323 c & 40.540 & - & 2.310 & - & - & - & Big PR \\
GJ 1132 & 0.180 & 2 & GJ 1132 c & 8.929 & - & 2.640 & - & - & - & Big PR \\
LHS 1140 & 0.180 & 2 & LHS 1140 b & 24.737 & 5.600 & - & 1.730 & 0.025 & - & Big PR \\
LHS 1140 & 0.180 & 2 & LHS 1140 c & 3.778 & 1.910 & - & 1.272 & 0.026 & - & Big PR \\
GJ 1132 & 0.190 & 2 & GJ 1132 b & 1.629 & 1.837 & 1.837 & 1.192 & 0.038 & - & Big PR \\
Kepler-1649 & 0.200 & 2 & Kepler-1649 b & 8.689 & - & - & 1.017 & 0.051 & 1.087 & Big PR \\
Kepler-1649 & 0.200 & 2 & Kepler-1649 c & 19.535 & - & - & 1.060 & 0.150 & 1.011 & Big PR \\
Kepler-446 & 0.220 & 3 & Kepler-446 b & 1.565 & - & - & 1.500 & 0.250 & 3.263 & Small PR \\
Kepler-446 & 0.220 & 3 & Kepler-446 c & 3.036 & - & - & 1.110 & 0.180 & 1.337 & Small PR \\
Kepler-446 & 0.220 & 3 & Kepler-446 d & 5.149 & - & - & 1.350 & 0.220 & 2.652 & Small PR \\
TOI-2096 & 0.230 & 2 & TOI-2096 b & 3.119 & - & - & 1.243 & 0.077 & 1.903 & Big PR \\
TOI-2096 & 0.230 & 2 & TOI-2096 c & 6.388 & - & - & 1.914 & 0.095 & 4.739 & Big PR \\
GJ 682 & 0.270 & 2 & GJ 682 b & 17.478 & - & 4.400 & - & - & - & Big PR \\
GJ 682 & 0.270 & 2 & GJ 682 c & 57.320 & - & 8.700 & - & - & - & Big PR \\
K2-72 & 0.270 & 4 & K2-72 b & 5.577 & - & - & 1.080 & 0.110 & 1.296 & Small PR \\
K2-72 & 0.270 & 4 & K2-72 c & 15.189 & - & - & 1.160 & 0.130 & 1.499 & Small PR \\
K2-72 & 0.270 & 4 & K2-72 d & 7.760 & - & - & 1.010 & 0.120 & 1.157 & Small PR \\
K2-72 & 0.270 & 4 & K2-72 e & 24.159 & - & - & 1.290 & 0.140 & 1.983 & Small PR \\
L 98-59 & 0.270 & 4 & L 98-59 b & 2.253 & 0.400 & - & 0.850 & 0.061 & - & Big PR \\
L 98-59 & 0.270 & 4 & L 98-59 c & 3.691 & 2.220 & - & 1.385 & 0.095 & - & Big PR \\
L 98-59 & 0.270 & 4 & L 98-59 d & 7.451 & 1.940 & - & 1.521 & 0.119 & - & Big PR \\
L 98-59 & 0.270 & 4 & L 98-59 e & 12.796 & - & 3.060 & - & - & - & Big PR \\
GJ 273 & 0.290 & 2 & GJ 273 b & 18.650 & - & 2.890 & - & - & - & Big PR \\
GJ 273 & 0.290 & 2 & GJ 273 c & 4.723 & - & 1.180 & - & - & - & Big PR \\
HIP 57274 & 0.290 & 3 & HIP 57274 b & 8.135 & - & 6.357 & - & - & - & Small PR \\
Wolf 1061 & 0.290 & 3 & Wolf 1061 b & 4.887 & - & 1.910 & - & - & - & Big PR \\
Wolf 1061 & 0.290 & 3 & Wolf 1061 c & 17.872 & - & 3.410 & - & - & - & Big PR \\
Wolf 1061 & 0.290 & 3 & Wolf 1061 d & 217.210 & - & 7.700 & - & - & - & Big PR \\
G 264-012 & 0.300 & 2 & G 264-012 b & 2.305 & - & 2.500 & - & - & - & Big PR \\
G 264-012 & 0.300 & 2 & G 264-012 c & 8.052 & - & 3.750 & - & - & - & Big PR \\
GJ 3929 & 0.310 & 2 & GJ 3929 b & 2.616 & 1.750 & - & 1.090 & 0.040 & - & Big PR \\
GJ 3929 & 0.310 & 2 & GJ 3929 c & 15.040 & - & 5.710 & - & - & - & Big PR \\
GJ 357 & 0.340 & 3 & GJ 357 b & 3.931 & - & - & 1.200 & 0.060 & 1.883 & Big PR \\
GJ 357 & 0.340 & 3 & GJ 357 c & 9.125 & - & 3.400 & - & - & - & Big PR \\
GJ 357 & 0.340 & 3 & GJ 357 d & 55.661 & - & 6.100 & - & - & - & Big PR \\
K2-239 & 0.400 & 3 & K2-239 b & 5.240 & - & - & 1.100 & 0.100 & 1.380 & Small PR \\
K2-239 & 0.400 & 3 & K2-239 c & 7.775 & - & - & 1.000 & 0.100 & 1.157 & Small PR \\
K2-239 & 0.400 & 3 & K2-239 d & 10.115 & - & - & 1.100 & 0.100 & 1.380 & Small PR \\
GJ 806 & 0.410 & 2 & GJ 806 b & 0.926 & 1.900 & - & 1.331 & 0.023 & - & Big PR \\
GJ 806 & 0.410 & 2 & GJ 806 c & 6.641 & - & 5.800 & - & - & - & Big PR \\
K2-316 & 0.410 & 2 & K2-316 b & 1.133 & - & - & 1.330 & 0.100 & 2.571 & Big PR \\
K2-316 & 0.410 & 2 & K2-316 c & 5.260 & - & - & 1.830 & 0.130 & 4.362 & Big PR \\
GJ 180 & 0.430 & 3 & GJ 180 b & 17.133 & - & 6.490 & - & - & - & Big PR \\
GJ 180 & 0.430 & 3 & GJ 180 c & 24.329 & - & 6.400 & - & - & - & Big PR \\
GJ 180 & 0.430 & 3 & GJ 180 d & 106.300 & - & 7.560 & - & - & - & Big PR \\
HD 260655 & 0.440 & 2 & HD 260655 b & 2.770 & 2.140 & - & 1.240 & 0.023 & - & Big PR \\
HD 260655 & 0.440 & 2 & HD 260655 c & 5.706 & 3.090 & - & 1.533 & 0.051 & - & Big PR \\
TOI-2095 & 0.440 & 2 & TOI-2095 b & 17.665 & 4.100 & - & 1.250 & 0.070 & - & Small PR \\
TOI-2095 & 0.440 & 2 & TOI-2095 c & 28.172 & 7.400 & - & 1.330 & 0.080 & - & Small PR \\
GJ 367 & 0.460 & 3 & GJ 367 b & 0.322 & 0.633 & - & 0.699 & 0.024 & - & Big PR \\
GJ 367 & 0.460 & 3 & GJ 367 c & 11.530 & - & 4.130 & - & - & - & Big PR \\
GJ 367 & 0.460 & 3 & GJ 367 d & 34.369 & - & 6.030 & - & - & - & Big PR \\
K2-83 & 0.480 & 2 & K2-83 b & 2.747 & - & - & 1.244 & 0.098 & 1.788 & Big PR \\
K2-83 & 0.480 & 2 & K2-83 c & 9.998 & - & - & 1.483 & 0.099 & 3.066 & Big PR \\
Kepler-186 & 0.480 & 5 & Kepler-186 b & 3.887 & - & - & 1.070 & 0.120 & 1.181 & Big PR \\
Kepler-186 & 0.480 & 5 & Kepler-186 c & 7.267 & - & - & 1.250 & 0.140 & 1.903 & Big PR \\
Kepler-186 & 0.480 & 5 & Kepler-186 d & 13.343 & - & - & 1.400 & 0.160 & 2.544 & Big PR \\
Kepler-186 & 0.480 & 5 & Kepler-186 e & 22.408 & - & - & 1.270 & 0.150 & 2.293 & Big PR \\
GJ 887 & 0.490 & 2 & GJ 887 b & 9.262 & - & 4.200 & - & - & - & Big PR \\
GJ 887 & 0.490 & 2 & GJ 887 c & 21.789 & - & 7.600 & - & - & - & Big PR \\
GJ 3998 & 0.500 & 2 & GJ 3998 b & 2.650 & - & 2.470 & - & - & - & Big PR \\
GJ 3998 & 0.500 & 2 & GJ 3998 c & 13.740 & - & 6.260 & - & - & - & Big PR \\
KOI-55 & 0.500 & 2 & KOI-55 b & 0.240 & 0.440 & - & 0.759 & - & - & Small PR \\
KOI-55 & 0.500 & 2 & KOI-55 c & 0.343 & 0.655 & - & 0.867 & - & - & Small PR \\
Kepler-138 & 0.540 & 4 & Kepler-138 b & 10.313 & 0.070 & - & 0.640 & 0.020 & - & Small PR \\
Kepler-138 & 0.540 & 4 & Kepler-138 c & 13.781 & 2.300 & - & 1.510 & 0.040 & - & Small PR \\
Kepler-138 & 0.540 & 4 & Kepler-138 d & 23.092 & 2.100 & - & 1.510 & 0.040 & - & Small PR \\
Kepler-138 & 0.540 & 4 & Kepler-138 e & 38.230 & 0.430 & - & - & - & - & Small PR \\
Kepler-186 & 0.540 & 5 & Kepler-186 f & 129.944 & - & - & 1.170 & 0.080 & 1.595 & Big PR \\
K2-240 & 0.580 & 2 & K2-240 b & 6.034 & - & - & 2.000 & 0.200 & 5.257 & Big PR \\
K2-240 & 0.580 & 2 & K2-240 c & 20.523 & - & - & 1.800 & 0.300 & 3.852 & Big PR \\
\bottomrule
\end{tabular}

    \begin{tablenotes}
      \small
      \item We first use the observed planet $m$ $M_{\oplus}$ if available.  If not, we then use the observed planet $m$sin$i$ $M_{\oplus}$, and if neither are available, we use the observed planet $r/R_{\oplus}$ with the upper error on the radii measurement ($+\sigma_1$ pl $r / R_{\oplus}$) to get the Approximate pl $m$ from FORECASTER.
    \end{tablenotes}

    
\end{table}

\end{turnpage}
\clearpage

==> response.tex <==
We thank Dan Tamayo for his time, for his helpful review, and for bringing to our attention the highly relevant literature that we have overlooked.  We have done our best to include all the key findings from the recommended literature.  We have also added emphasis that the new findings here are the specific prediction of the presence of a period ratio greater than two in a multi-planet M-dwarf system to be a signature of a late stage instability, thus allowing us to identify the systems that likely experienced late stage giant impacts on at least some of their planets.  We have also added in some details about the differences in multiplicities between our simulated sets and the observations that we initially overlooked.  We show all changes to the manuscript in red text.

Reviewer:
The authors take a previously published suite of integrations simulating the formation of TRAPPIST-1 analogues and integrate them from the time of disk dissipation at 3 Myr out to 100 Myr, finding that about half of them undergo collisions or ejections post-disk dispersal. The authors explore both criteria that might separate the initial conditions that eventually go unstable from ones that do not, and look for observational signatures in the systems that go unstable that could separate them from ones that remain stable. They argue from from the wide period separations in observed planetary systems that approximately 75% of systems around M-dwarfs have undergone dynamical instabilities.

I believe the results will be of interest to AAS journal readers, and I am very happy to recommend its publication following the consideration of the mostly minor comments below. None of them are major issues, so the authors should feel free to incorporate them as they see fit.

Dan Tamayo

Broader Comments:

It would seem valuable to discuss some of the uncertainties introduced by our incomplete understanding of the planet formation process, and qualify some of the conclusions in that context. Specifically, The paper makes a strong case that if planetary systems form around M-dwarfs through pebble accretion and by piling up planets into resonant chains starting at the disk's inner edge, then one can separate systems that underwent instabilities from ones that didn't by looking for period ratios > 2. But can we be confident that this is the right formation picture? Couldn't MMR chains and wider separation systems represent different formation pathways? Certainly observed resonant chains would seem to require migration, but there's also been a lot of work looking at in-situ formation without forming resonant chains (Hansen & Murray 2012, 2013, Dawson et al. 2016 and many others). Should it give us pause that in the one case where we have strong geochemical evidence for early collisions (the inner solar system), we seem to have an edge case with period ratios mostly < 2? Not saying every sentence needs to be qualified by three clauses, but some discussion of this might be valuable up front to frame the investigation.

RESPONSE: Yes, in situ accretion would be likely to result in the same 'unstable characteristics' we identify here, such as period ratios larger than two like we see with Mercury and Venus.  You bring up a good point that we cannot differentiate between systems that formed primarily through pebble accretion and went unstable, and systems that formed primarily through late stage core accretion. We add a mention to this in the introduction and a discussion of this to Section 6.

It also seemed to me like there could be ways in which the paper could better guide the reader  up front on the aspects of the simulations that matter the most. For example, the paper starts by discussing how 28 of the systems started with 6+ planets, and 72 with < 6. I was distracted by the fact that surely this breakdown depends significantly on several model assumptions used in paper I. This would be a problem if trying to explain the prevalence of TRAPPIST-1 like systems, but presumably the 28-72 split doesn't matter a lot to the eventual conclusion of the paper that if closely packed systems go unstable, this will tend to lead to period ratios > 2. I want to emphasize that I think the sections breaking down the commonalities among systems that went unstable were very valuable, but I think it could help the reader to provide some big picture context discussing that e.g. the synthetic systems generated in this way will be model dependent with uncertain parameters, that that shouldn't matter much for the conclusions of the paper, and that it's interesting to nevertheless dig down into the particulars of the distribution in this set of runs to help clarify what caused some of them to be unstable.

RESPONSE: We have removed references to the specific findings of the results of paper I and agree that producing T1 analogs is model dependent.  We have tried to restructure the introduction to make it more clear that we are interested in observational signatures of systems that formed in resonant chains and experienced an instability after gas disk dissipation.

How is the damping turned off at 3 Myr to integrate for the 100 Myr? One thing that we found in our TRAPPIST-1 simulations (https://ui.adsabs.harvard.edu/abs/2017ApJ...840L..19T/abstract) was that the way we did this made a big difference to the results. Specifically, especially in cases with strong eccentricity damping, the effect induces changes in both the equilibrium resonant angle and equilibrium eccentricity. So when the effect is turned off discretely, the system is now off the equilibrium value and oscillates with wider amplitude around the equilibrium (which makes things more unstable). By contrast, if the effects are turned off slowly to (presumably) mimic the dissipation of the disk, the system adiabatically ends up in the gas-free equilibrium configuration oscillating with small amplitudes. We found this leads to significantly improved stability. Note: Found this in the last paragraph. I think this would be helpful in the methods section for the reader to be able to interpret the results. This is another example where the type of framing mentioned above might help. If the goal were to faithfully obtain what fraction of systems go unstable this would be a problem--but if the question is trying to understand what systems look like post-instability, this probably doesn't matter. In fact, maybe it helps by causing more instabilities to improve the statistics for the U sample?

RESPONSE:  We apologize for overlooking your paper.  We have tried to clarify the goal of the paper in the introduction to avoid confusion and to be consistent with the findings of your paper.

Specifics 

These references seemed important to include in the context of resonant chains going unstable:
https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1750I/abstract
https://ui.adsabs.harvard.edu/abs/2021A%26A...650A.152I/abstract
https://ui.adsabs.harvard.edu/abs/2017ApJ...840L..19T/abstract
https://ui.adsabs.harvard.edu/abs/2022AJ....163..201G/abstract

RESPONSE:  Indeed, these papers are highly relevant.  We add the first three papers to the discussion in the context of our findings and reference your paper in the introduction.

L644 Previous studies suggested secular instabilities, here we show that short-term instabilities can also be the culprit. Possibly useful theoretical references:
This paper studied why resonant chains might go unstable, but found that instabilities typically occurred at higher planet masses ~ 1 MJup: https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.4950P/abstract

These papers argue that the short instability times are due to the faster effects of mean motion resonances (compared to secular resonances):

Our paper shows that resonant regions become chaotic due to the secular eccentricity variations periodically sweeping the chaotic edges of MMRs to wider and narrower period ratios: https://ui.adsabs.harvard.edu/abs/2021AJ....162..220T/abstract

These papers argue that instabilities in closely packed systems can also be driven by the overlap of 3-body resonances:

https://ui.adsabs.harvard.edu/abs/2011MNRAS.418.1043Q/abstract
https://ui.adsabs.harvard.edu/abs/2020A%26A...641A.176P/abstract
https://ui.adsabs.harvard.edu/abs/2022ApJ...932...61R/abstract

RESPONSE:  We have added all the above references to the introduction.

L212 / L224: Why are there 24 T1 analogues, but column 1 for T1A is 28? If it's the different definition of a planet, it might be helpful to move those statements starting in line 224 up here. If not, why is that?

RESPONSE:  Yes, it is because of the different definitions we adopt for a planet.  We have removed the sentence in Section 2 that summarizes the findings from paper I, and the mention of 24 planets,  as it is tangent to this paper.

Sec 2: I had trouble parsing the different groups on a first read. I think it would have helped me to start the description with the first column of Table 1. If I understood correctly: out of our 100 simulations 28 formed 6+ planets, and 72 formed <6. And then to break it up into final outcomes, e.g. both categories could go unstable and contribute to U, and the stable ones go into T1A and PLM respectively.

RESPONSE: Yes this is correct.  We have restructured the table accordingly and clarified the groups in the table caption.

L308: By contrast, the U runs exhibit more period ratios that are not near significant MMRs. My (wrong) immediate reaction to this was that of course unstable systems would be left with fewer MMRs--maybe it could help to specify 'the initial conditions that undergo instability after disk dissipation (U systems) exhibit more period ratios that are not near significant MMRs.' It also might help to say what fraction? It seems roughly from Fig 1 like it's still a minority? ~20-30% of U systems (?)

RESPONSE:  This has been rephrased and the fraction of U systems that are not near an MMR has been input.

L346: Counterintuitively, the U systems have lower AMD than others. It wasn't clear to me that a slightly higher eccentricity damping for U systems could explain this difference. Is it possible to rule out either of these possibilities?

I couldn't tell from the introduction what migration and eccentricity damping prescriptions were used (it might be worth mentioning). If these do boil down to prescriptions that induce exponential eccentricity and semimajor axis damping, then the equilibrium eccentricity planets should reach in a j:j-1 MMR is given by e_eq = (tau_e / (3(j+1)tau_a)^{1/2} e.g. eq 24 of https://iopscience.iop.org/article/10.1088/0004-6256/147/2/32/meta. So the fact that U systems have stronger eccentricity damping further in wouldn't explain the lower eccentricities unless tau_a changed in a different way (in Goldreich & Schlichting they keep a ratio of K=tau_a/tau_e ~ 100). But if you are maintaining the same ratio of tau_e to tau_a in your prescription (so their Eq 24 applies), then perhaps that gives a more direct explanation--that because the U systems are closer together and in first-order MMRs with higher j, the equilibrium eccentricity is lower. 

Alternatively, planet pairs in MMRs will damp to a non-zero forced eccentricity while non-resonant systems will damp to 0. Could it just be that if U systems have 30% fewer pairs of planets in MMRs, these planet pairs get damped to 0 eccentricity so the overall population has a lower AMD?

It seems like both these effects could plausibly contribute, and understanding them in the initial conditions could help interpret the outcomes? Perhaps splitting the U population into two according to whether all pairs are in resonances or not and comparing those two subpopulations to T1A and PLM could help disentangle which of these matter most? Maybe both do?

RESPONSE:  Our prescriptions for eccentricity and semi-major axis are from Tanaka et al. 2002. We have added all the citations for the prescriptions we used in Paper I to the introduction. Performing your suggested test, we find that the systems without a resonance have much lower eccentricities than all the other systems that contain only MMRs confirming that it is the absence of MMRs that is contributing to the low eccentricity. When considering the eccentricities of the planets in the U runs that have all MMRs and similarly for the PLM runs, we do not find that the U planets have a lower eccentricity thus ruling out contributions from dynamical spacing.  We thank you for bringing this to our attention and have updated our explanation for the lower AMD of the U systems accordingly.

L242: Are ejections common? This is discussed at the end of this subsection, but this statement seemed surprising given the parameters at the start of Sec 2. Would it make sense to move that sentence to where it's discussed and possibly expanding on it?, e.g.,  Because the escape speed from these planets is typically slower than their orbital velocities, interplanetary collisions are much more common than ejections (e.g., Petrovich et al. 2014). However, we track both and observe ejections in 5 out of our 100 simulations. 

@article{petrovich2014scattering, title={Scattering outcomes of close-in planets: constraints on planet migration}, author={Petrovich, Cristobal and Tremaine, Scott and Rafikov, Roman}, journal={The Astrophysical Journal}, volume={786}, number={2}, pages={101}, year={2014}, publisher={IOP Publishing}}

RESPONSE:  No. Ejections are not common and we have made the recommended change in the beginning of Section 3.

Appendix A seems to be missing

RESPONSE:  We have opted to remove the appendix and include the observational data tables in the main text.
